Streamflow Prediction with Uncertainty Quantification for Water Management: A Constrained Reasoning and Learning Approach

Predicting the spatiotemporal variation in streamflow along with uncertainty quantification enables decision-making for sustainable management of scarce water resources. Process-based hydrological models (aka physics-based models) are based on physical laws, but using simplifying assumptions which can lead to poor accuracy. Data-driven approaches offer a powerful alternative, but they require large amount of training data and tend to produce predictions that are inconsistent with physical laws. This paper studies a constrained reasoning and learning (CRL) approach where physical laws represented as logical constraints are integrated as a layer in the deep neural network. To address small data setting, we develop a theoretically-grounded training approach to improve the generalization accuracy of deep models. For uncertainty quantification, we combine the synergistic strengths of Gaussian processes (GPs) and deep temporal models (i.e., deep models for time-series forecasting) by passing the learned latent representation as input to a standard distance-based kernel. Experiments on multiple real-world datasets demonstrate the effectiveness of both CRL and GP with deep kernel approaches over strong baseline methods.

==> Figures/figCorrelations.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/Annual_correlation_3vars_V8.jpeg}
\vspace{-0.35in}
  \caption{\small Correlation between errors (ranked low to high)  environmental variables (ranked low to high). 
  \label{fig:correlation}
  }
\end{figure}


==> Figures/figPerfChart.tex <==
\begin{figure}[H]
  \centering
  \includegraphics[width=0.4\textwidth]{Figures/Performance_chart_flathead_V8.jpeg}
\vspace{-0.175in}
  \caption{\small Relative performance chart comparing all models for Flathead watershed. For each test month, each model's MAE was compared against the best performing model's MAE for that month (difference shown in X-axis). The fraction of test months for which that performance is achieved is shown along Y-axis. Closer a curve is aligned with the Y-axis for larger fraction, the better.
    \label{fig:performance}
  }
\end{figure}

==> Figures/tableMAE.tex <==
\begin{table}[ht]
\begin{tabular}{llllll}
\hline
\rowcolor[HTML]{C0C0C0}
\textbf{} & 
{\small {\begin{tabular}[c]{@{}l@{}}\hspace{-0.1in} VIC- \\ \hspace{-0.07in}CropSyst\end{tabular}}} &  
{\small \hspace{-0.1in} {RCGNN}} & 
{\small {\begin{tabular}[c]{@{}l@{}} \hspace{-0.1in} PG- \\\hspace{-0.1in} RCGNN\end{tabular}}} & 
{\small {\begin{tabular}[c]{@{}l@{}}\hspace{-0.1in} RCGNN \\ \hspace{-0.1in} -NSL\end{tabular}}} & 
{\small {\begin{tabular}[c]{@{}l@{}} { \hspace{-0.1in} RCGNN \\ \hspace{-0.1in} -NSL-IW } \end{tabular}} }
\\\hline
{\small BR} \hspace{0.0in} & {0.55}  & {0.42} & {\textbf{0.41}} & {0.46} & {{0.44} \\ 
\rowcolor{aliceblue} 
{\small C} \hspace{-0.0in} & {0.41} & {0.41} & {0.50} & {0.37} & {\textbf{0.36}} \\ 
{\small CCR} \hspace{-0.0in} & {0.77} & {0.64} & {1.07} & {1.23} & {\textbf{0.61}} \\ 
\rowcolor{aliceblue} 
{\small F} \hspace{-0.0in} & {1.07} & {1.14} & {0.78} & {0.77} & {\textbf{0.62}} \\ 
{\small SFC} \hspace{-0.0in} & {0.26}& {0.22}& {0.21}& {0.22}& {\textbf{0.21}}\\ 
\rowcolor{aliceblue} 
{\small Y} \hspace{-0.0in} & {0.37}& {0.20}& {0.20}& {0.20}& {\textbf{0.18}}\\ \hline
\toprule
\end{tabular}
\vspace{-0.125in}
\caption{Comparison of predictive models across watersheds. The MAE (lower the better) is measured in mm.
\label{tab:MAE_comparison}
}
}
\end{table}

==> Figures/table_NNSE_low_flow.tex <==
\begin{table}[H]
\begin{tabular}{p{0.5cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}}
\hline
\textbf{} & 
{\small {\begin{tabular}[c]{@{}l@{}}VIC- \\ CropSyst\end{tabular}} }& 
{\small {RCGNN} }& 
{\small {\begin{tabular}[c]{@{}l@{}}PG- \\ RCGNN \end{tabular}}} & 
{\small {\begin{tabular}[c]{@{}l@{}}RCGNN- \\ CRL\end{tabular}}} & 
{\small \hspace{-0.1in} {\begin{tabular}[c]{@{}l@{}}RCGNN- \\ CRL-IW\end{tabular}}} \\ \hline
BR & 0.9337 & 0.5828 & 0.5718 & 0.5788 & 0.5934 \\
C &0.9599 &0.6766 &0.6391 &0.6892 & 0.7082 \\
CCR &0.8938 &0.6777 &0.6668 &0.7658 & 0.7752 \\
F  &0.9707 &0.4709 &0.5162 &0.5985 &0.6638 \\
SFC &0.9363 &0.5144 &0.581 &0.6292 &0.6569 \\ 
Y  &0.3506 &0.1099 &0.1579 &0.2397 &0.2549 \\ \hline
\toprule
\end{tabular}
\vspace{-0.01in}
\caption{\small Comparison of predictive models across watersheds during low flow months. Values are reported in terms of the NNSE metric (higher the better).
NNSE values less than 0.5 indicate that the mean is a better predictor than the model's output.
}
\label{tab:NNSE_comparison_low_flow}
\end{table}




\iffalse
\begin{table}[H]
\begin{tabular}{c|ccccc} 
\hline
                         & VIC-CropSys        & RCGNN        & PG-RCGNN   & RCGNN-NSL    & RCGNN-NSL w/ IW \\ \hline
BR              & 0.7812 & 0.7955 & 0.7969 & 0.8003 & \textbf{0.8069} \\
C               & 0.8458 & 0.8489 & 0.8247 & 0.8737 & \textbf{0.9007} \\
CCR & 0.8241 & 0.8175 & 0.8140 & 0.7944 & \textbf{0.8788} \\
F                 & 0.7178 & 0.7334 & 0.7826 & 0.8032 & \textbf{0.8908} \\
SFC    & 0.7928 & 0.8177 & 0.7724 & 0.8177 & \textbf{0.8580} \\
Y                   & 0.255  & 0.3092 & 0.2673 & 0.3822 & \textbf{0.4705} \\
\hline
\end{tabular}
\caption{Comparison of models across watersheds. Abbreviations: VIC (Variable Infiltration Capacity model), GNN (Graph Neural Network), GNN+Loss (Graph Neural Network with Loss), GNN+NSL (Graph Neural Network with neuro-symbolic learning), GNN+NSL+IW (Graph neural network with neuro-symbolic learning and importance weighted training). Values are reported in terms of the NNSE (Normalized Nash–Sutcliffe Efficiency ) metric.}
\label{tab:NNSE_comparison}
\end{table}
\fi

==> Figures/table_constraint_fraction.tex <==
\begin{table}[H]
\begin{center}
\begin{tabular}{lll}
\toprule
    & PG-RCGNN & RCGNN-RCL-IW \\
\hline
BR  & 0.44 & 0 \\
C   & 0.44 & 0 \\
CCR & 0.44 & 0 \\
F   & 0.67 & 0 \\
SF  & 0.11 & 0 \\
Y   & 0 & 0 \\
\hline
\label{tab:constraint_fraction}
\end{tabular}
\caption{\small Comparison of yearly constraint violation fractions during test years.}
\end{center}
\end{table}

==> Figures/table_constraint_magnitude.tex <==
\begin{table}[H]
\begin{center}    
\begin{tabular}{lll}
\toprule 
    & PG-RCGNN & RCGNN-RCL-IW \\
\hline
BR  & 51.41 & 0 \\
C   & 25.93 & 0 \\
CCR & 106.1 & 0 \\
F   & 52.26 & 0 \\
SF  & 8.09 & 0 \\
Y   & 0 & 0 \\
\hline
\label{tab:constraint_magnitude}
\end{tabular}
\caption{Comparison of yearly constraint violation magnitudes (averaged across all the test years). The values are reported in mm.}
\end{center}
\end{table}

==> Figures/table_dropout.tex <==
\begin{table}[H]
\begin{center}
\begin{tabular}{lllllll}
\hline
\multirow{2}{*}{} & \multicolumn{6}{c}{dropout rates}                                           \\
                  & \multicolumn{2}{c}{0.2} & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{0.5} \\
                  & coverage   & PI width   & coverage   & PI width   & coverage   & PI width   \\
\hline
BR  & 74.07 & 4.77 & 76.85 & 7.83 & 81.48 & 11.51\\
C  & 76.85 & 4.7 & 78.7 & 7.67 & 83.33 & 12.21 \\
CCR & 79.62 & 5.47 & 81.48 & 7.74 & 85.18 & 11.45\\
F & 75.92 & 4.92 & 78.7 & 7.98 & 83.33 & 12.37\\
SF & 78.7 & 4.59 & 81.48 & 7.61 & 86.11 & 12.78\\
Y & 81.48 & 4.37 & 83.33 & 6.89 & 87.03 & 12.35\\
\hline
\end{tabular}
\caption{\small Comparison of coverage and prediction interval width with dropout across various dropout rates}
\label{tab:dropout}
\end{center}
\end{table}
